Nl2Hltl2Plan: Scaling Up Natural Language Understanding for Multi-Robots Through Hierarchical Temporal Logic Task Representation

To enable non-experts to specify long-horizon, multi-robot collaborative tasks, language models are increasingly used to translate natural language commands into formal specifications. However, because translation can occur in multiple ways, such translations may lack accuracy or lead to inefficient multi-robot planning. Our key insight is that concise hierarchical specifications can simplify planning while remaining straightforward to derive from human instructions. We propose Nl2Hltl2Plan, a framework that translates natural language commands into hierarchical Linear Temporal Logic (LTL) and solves the corresponding planning problem. The translation involves two steps leveraging Large Language Models (LLMs). First, an LLM transforms instructions into a Hierarchical Task Tree, capturing logical and temporal relations. Next, a fine-tuned LLM converts sub-tasks into flat LTL formulas, which are aggregated into hierarchical specifications, with the lowest level corresponding to ordered robot actions. These specifications are then used with off-the-shelf planners. Our Nl2Hltl2Plan demonstrates the potential of LLMs in hierarchical reasoning for multi-robot task planning. Evaluations in simulation and real-world experiments with human participants show that Nl2Hltl2Plan outperforms existing methods, handling more complex instructions while achieving higher success rates and lower costs in task allocation and planning. Additional details are available at https://nl2hltl2plan.github.io .

==> preliminary.tex <==
\section{Hierarchical Linear Temporal Logic}\label{sec:preliminaries}
% \subsection{Hierarchical Task Network}
% Hierarchical Task Network (HTN) is a framework used to decompose and organize complex tasks for which are naturally organized hierarchy. It breaks down complex tasks into simpler, more manageable sub-tasks with partial-order, forming a hierarchy of primitive actions and non-primitive actions. The classic HTN deduce and expand tasks until each sub-tasks of any non-primitive actions are primitive operators.
% It would be a waste of time to construct a flat LTL, using a build-in hierarchy help escape from the exponential explosion.
% {\color{red} do we need to explain this?}
% \paragraph{Linear Temporal Logic}
Linear Temporal Logic (LTL) is composed of basic statements, referred to as atomic propositions $\mathcal{AP}$, along with boolean operators such as conjunction ($\wedge$) and negation ($\neg$), and temporal operators like next ($\bigcirc$) and until ($\mathcal{U}$)~\cite{baier2008principles}. LTL formulas follow the syntax:
% \begin{align}\label{eq:grammar}
    $\phi:=\top~|~\pi~|~\phi_1\wedge\phi_2~|~\neg\phi~|~\bigcirc\phi~|~\phi_1~\mathcal{U}~\phi_2$, 
% \end{align}
where $\top$ stands for a true statement, and $\pi$ is a boolean valued atomic proposition. Other temporal operators can be derived from $\mathcal{U}$, such as $\Diamond \phi$ that implies $\phi$ will be true at a future time.
% An infinite {\it word} $w$ over the alphabet $2^{\mathcal{AP}}$, where $\mathcal{AP}$ is the set of atomic propositions, can be denoted as $w=\sigma_0\sigma_1\ldots\in (2^{\mathcal{AP}})^{\omega}$, with $\omega$ signifying infinite repetition, and $\sigma_k\in2^{\mathcal{AP}}$ for $
% \forall k\in\mathbb{N}$. The {\it language} $\texttt{Words}(\phi)$ is the collection of words that meet the formula $\phi$. This means, $w$ belongs to $\texttt{Words}(\phi)$ if and only if $w\models\phi$. The satisfaction relation, represented by $\models$, pairs elements from $(2^{\mathcal{AP}})^{\omega}\times\phi$.
We focus on a subset of LTL known as syntactically co-safe formulas (sc-LTL)~\cite{kupferman2001model}. Any LTL formula encompassing only the temporal operators $\Diamond$ and $\mathcal{U}$ and written in positive normal form (where negation is exclusively before atomic propositions) is classified under sc-LTL formulas~\cite{kupferman2001model}, which can be satisfied by finite sequences followed by any infinite repetitions. This makes sc-LTL apt for reasoning about robot tasks with finite durations.


==> tasks/ai2-thor.tex <==
\section{AI2-THOR}\label{app:ai2thor}
\subsection{Generation of derivative tasks}\label{app:generation_derivative_tasks}
We create larger tasks by merging a specific number of base tasks, introducing various temporal constraints to these combinations, which we refer to as \textit{derivative} tasks. Specifically, to ensure that the same object is not included in multiple base tasks simultaneously, we first use an LLM to identify the objects involved in each base task. We then combine base tasks that involve distinct objects and randomly establish temporal relationships between them. Subsequently, an LLM reformulates this randomly combined information into derivative tasks that align more naturally with human expression patterns. 
% \subsection{Derivative tasks with 4 base tasks}
\label{app:derivative_tasks}
 \href{https://nl2hltl.github.io/prompts/aithor-4basetask.html}{Here is a list of these derivative tasks with 4 base tasks}
\label{fig:instruction_sim_4base_task}.
% \subsection{2 base tasks}
% \subsection{3 base tasks}
% \subsection{Derivative tasks with 4 base tasks}

% \begin{enumerate}
%     % \item Pick up the keys near the lamp to turn it off. After turning off the lamp, move the computer from the table to the chair. Simultaneously, take the box from the dining table and put it on the red couch. Lastly, Pick up a watch from the table, one-at-a-time, and put them on the TV stand.
%     \item Put a microwaved egg in the garbage can. Place a rinsed spoon into the drawer. Heat up a slice of potato and put it against the apple. After these are finished, put the tomato in the microwave.
%     \item First Rinse off a tomato slice and cook it in the microwave. Next, heat and place a potato in the sink. Then, put the statue in the sink. Finally, place a heated mug on a counter.
%     \item Put a bowl with a credit card on the table at any time. Meanwhile place the watch on the table on a plate in any order. After placing the bowl and the watch, put the box with vase in it beside the laptop on the table. Finally, place newspaper onto the sofa.
%     \item Place a credit card inside a box and take the box to a shelf. At same time, take the remote controls and place them on the couch. After completing these tasks, move a pillow from the couch to a chair. Finally, place a plate with key chain on it on the table in the corner of the room.
%     \item Move the plunger to the cabinet under the sink at any time. Put the soap bottle on top of the toilet at any time. in any order, put a towel on the toilet at any time. After placing the plunger, soap bottle, and towel, put a bar of soap on the back of the toilet.
%     \item Get spray bottle from toilet, place spray bottle on dresser at any time. After that, place a clean bar of soap down on top of the toilet. Once done, store a plunger in a  dresser. Lastly, put away candles in the cabinet.
%     \item Pick up the key chain near the lamp to turn it off. After turning off the lamp, move the laptop from the table to the chair. At any time, take the box from the table and put it on the couch. Lastly, Pick up a watch from the table,  and put them on the TV stand.
%     % \item Place statues on the table at any time. Simultaneously, put a box containing a credit card on the couch. After placing the statues, move keys and a plate to the coffee table. Finally, examine a watch by the light of a floor lamp.
%     % \item Place a warmed glass in the sink at any time. Simultaneously, drop a cooked egg in the sink. After dropping the egg, put a couple of pepper grinders in the kitchen cabinet.Then put the knife in the drawer.
%     % \item Slice the bread, cook a slice, and put it on the table at any time. Simultaneously, put a cold egg on the counter and place a chilled bowl in a cabinet. After placing the bowl, put the chilled slice potato in the sink.
%     % \item Place a cooked apple inside the fridge at any time. Simultaneously, put a chilled tomato in the microwave. After placing the apple, put a fork in a pan plus move it to the left side counter. Finally, place the rinsed green cup filled with water back into the microwave.
% \end{enumerate}

% \subsection{Simulation results}\label{app:sim_res}

% \begin{figure}[!t]
%     \centering
%     \includegraphics[width=\linewidth]{demo/demo.png}
%     \caption{A series of snapshots for task ``First Put the clean spatula in the drawer and put a pepper shaker in the kitchen cabinet in any order. After putting the spatula and the pepper shakers, rinse an apple to put it in the microwave. Finally, wash the spoon on the counter and place it on a plate'' (the spatula and its movement is highlighted by green mask, the pepper shaker and its movement is highlighted by orange mask, the apple and its movement is highlighted by red mask, and the spoon and its movement is highlighted by yellow mask).}
%     \label{fig:ai2thor}
% \end{figure}




==> tasks/real-world.tex <==
\section{Real-world experiments}\label{app:real-world-exp}
% \begin{table*}[!tbh]
%     \centering
%     \begin{tabular}{p{7cm}p{7cm}}
%     \bhline
%     task description & { paraphrase} \\
%     \hline
%        % \multirow{4}{7cm}{First place the red apple, then the green apple, and finally the orange onto the yellow plate.}  & 1. Put red apple, the green apple and the orange into the red plate.\\
%        % & 2. I would you to move the red apple, then the green apple and lastly orange to the yellow plate.\\
%        % & 3. Please put the red apple, green apple, and orange onto the yellow plate in this order.\\
%        % & 4. Sequentially, firstly put red apple into a yellow plate , and then put green apple into a yellow plate , and finally put the orange into a yellow plate\\
%        % \hline
%          \multirow{4}{7cm}{5. Simultaneously place the green apple in the blue plate and the orange in the yellow plate.}  & 1. Put the green apple to the blue plate and the orange to the yellow plate. The order does not matter.\\
%        & 2. Please put the green apple into the blue plate and orange into the yellow plate in any order.\\
%        & 3. Please place the green apple in the blue plate and the orange in the yellow plate at the same time.\\
%        & 4. You can put the green apple in to the blue plate and the orange into the yellow plate in any order.\\
%        \hline
%          \multirow{4}{7cm}{6. Place the green apple in the pink plate, the orange in the yellow plate and the red apple in the blue plate. The order of placement is not specified and can be chosen freely.}  & 1. Put the green apple to the pink plate, the orange to the yellow plate and the red apple to the blue plate in any order.\\
%        & 2. Please put the green apple in the pick plate, the orange in the yellow plate and red apple int he blue plate. I do not care about the order.\\
%        & 3. Please place the green apple in the pink plate, the orange in the yellow plate, and the red apple in the blue plate. In any order you prefer.\\
%        & 4. a.place the green apple into the pink plate b. put the orange into the yellow plate c. put the red apple in the blue plate. a and b and c can be done in any order \\
%        \hline
%          \multirow{4}{7cm}{7. Place the carrot in the blue plate, the orange in the yellow plate, the green apple in the green plate, and the red apple in the pink plate in any order.}  & 1. Put the carrot to the blue plate the orange to the yellow plate the green apple to the green plate and the red apple to the pink plate in the best order.\\
%        & 2. I want the carrot to be in the blue plate, the orange in the yellow plate, the green apple in the green plate. The order is not important.\\
%        & 3. Place the carrot in the blue plate, the orange in the yellow plate, the green apple in the green plate, and the red apple in the pink plate. You can decide the order freely. \\
%        & 4. Place the carrot in the blue plate in any order, the orange in the yellow plate in any order, the green apple in the green plate in any order, and the red apple in the pink plate in any order. all the tasks should be finished in the end\\
%        \hline
%          \multirow{4}{7cm}{8. Begin by placing the green apple and orange in the yellow plate in any order. Once done, place the carrot and red apple in the blue plate also in any order.}  & 1. First put the green apple and the orange to the yellow plate, and then put the place the carrot and the red apple to the blue plate in the best order.\\
%        &  2. Start placing the green apple and orange in the yellow plate in any order. After that, then put the carrot and red apple in the blue plate in any order.\\
%        & 3. Please place place the green apple and orange in the yellow plate in any order. Then place the carrot and red apple in the blue plate in any order.\\
%        & 4. First place the green apple and an orange into a yellow plate in any order. after that, place the carrot and the red apple into a blue plate in any order, too. \\
%          \bhline
%     \end{tabular}
%     \caption{A collection of representative tasks along with their rephrasings.}
%     \label{tab:real-world-rephrase}
% \end{table*}
\href{https://nl2hltl.github.io/prompts/real_world_task_1.html}{A collection of representative tasks along with their rephrasings}
\label{tab:real-world-rephrase}
% \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.8\linewidth]{figs/real_world1.png}
%     \caption{Experimental Setup in a Real-World Environment.}
%     \label{fig:real-world-setup}
% \end{figure}

\href{https://nl2hltl.github.io/prompts/Prompt_for_LLMs.html}{Prompt for LLMs to generate task plan}
\label{fig:Prompt_for_LLMs}
% \begin{tcolorbox}[breakable,title=Prompt for LLMs to generate task plan]% \tcblower
% Given a tabletop scenario with various fruits and vegetables, and colored plates, a robotic arm is tasked to arrange these items according to instructions. The initial coordinates of each fruit, vegetable, and the robotic arm are provided. Using the available information and predefined API functions like \texttt{pickup(object)} and \texttt{place(object, target)}, generate a sequence of commands to effectively arrange each item on the correct colored plate.\\

% API: 
% \begin{verbatim}
% move_to(obj) 
% pickup(obj) 
% move_to(plate) 
% release_obj(plate)
% \end{verbatim}\\
% \vspace{1em}

% Initial coordinates: \\
% apple: (1, 2) \\
% banana: (3, 4) \\
% orange: (5, 6) \\
% carrot: (7, 8) 
% \vspace{1em}

% Task: 
% Considering the initial coordinates, output a sequence of API calls to complete the task so that the trajectory of the robot arm has the lowest cost. Make sure that that job can be completed with the objects in the environment. Make sure the environment has all the objects and plates that are mentioned in the task. If the task is not possible, please output `Invalid input'. If the task can be planned, just output the sequences of API calls in the following format: 
% Plan: 1. xxx 2.xxx 
% \vspace{1em}

% Example: \\
% Input: Place the xxx in the aaa plate and the yyy in the bbb plate. \\
% Output should be like the following:

% \begin{verbatim}
% Plan: 
% 1. move_to(xxx)
% 2. pickup(xxx)
% 3. move_to(aaa_plate)
% 4. release_obj(aaa_plate)
% 5. move_to(yyy)
% 6. pickup(yyy)
% 7. move_to(bbb_plate)
% 8. release_obj(bbb_plate)
% \end{verbatim}

% Here is the task input:  Place the apple in the red plate and the banana in the yellow plate. 
% % \tcblower
% \end{tcolorbox}
% \begin{figure}[H]
%     \caption{Prompt for LLMs to generate task plan}
%     \label{fig:Prompt_for_LLMs}
% \end{figure}





\href{https://nl2hltl.github.io/prompts/Prompt_for_multi-robot-LLMs.html}{Prompt for LLMs to generate multi-robot handover task plan}
\label{fig:Prompt_for_multi-robot-LLMs}
% \begin{tcolorbox}[breakable,title=Prompt for LLMs to generate multi-robot handover task plan]% \tcblower
% {\color{\modifycolor}We have arms $a, b, c$ and $d$. The distance between each robotic arm is 1 meter, each robot arm has a motion radius of 0.8 meters that means each arm can only pick and place the object in the regions besides them. Each goal region can only place one object. 

% API: 
% \begin{verbatim}
% pick(arm_id, object_i, place_j)
% drop(arm_id, object_i, place_j)
% handover(arm_id_i, amd_id_j)
% \end{verbatim}\\
% \vspace{1em}

% Initial coordinates 
% % (or given by image token <img Fig. \ref{fig:multi_arm_handover-line} Fig.\ref{fig:multi_arm_handover-square}>)
% : 

% arm $a$ at (0, 0),

% arm $b$ at (0, 1), 

% arm $c$ at (-1, 1), 

% arm $d$ at (-1, 0), 

% block $a$ at region $E$ (0.2, 0) 

% block $b$ at region $F$ (0.2, 0.5), 

% block $c$ at region $G$ (0.2, 1).

% Goal region:

%     region $J$ at (-1.2, 0), 
    
%     region $H$ at (-1.2, 0.5), 
    
%     region $I$ at (-1.2, 1)
% \vspace{1em}

% Task: Considering the initial coordinates, output a sequence of API calls to complete the task so that the trajectory of the robot arm has the lowest cost. Make sure that that job can be completed with the objects in the environment. Make sure the environment has all the objects and plates that are mentioned in the task. If the task is not possible, please output `Invalid input'. If the task can be planned, just output the sequences of API calls in the following format: 
% Plan: 1. xxx 2.xxx 
% \vspace{1em}

% Here is the task input: Please place the blue block into region I, the red block into region J, the yellow block into region H. Place the red block before placing the blue block. }
% . 
% % \tcblower
% \end{tcolorbox}
% \begin{figure}[H]
%     \caption{Prompt for LLMs to generate task plan for multi-robot handover task}
%     \label{fig:Prompt_for_multi-robot-LLMs}
% \end{figure}




% {\color{\modifycolor}
% \begin{figure}[!t]
%     \centering
%     \includegraphics[width=0.6\linewidth]{figs/four_robot_close_three_object_hand_over-2.png}
%     \caption{Four-robot-in-square scene diagram of multi robot collaboration as image prompt transmitted to LLM planner. (the distance between each robot arm is 1m, and each arm's motion radius is about 0.8m)}
%     \label{fig:multi_arm_handover-square}
%     \vspace{-10pt}
% \end{figure}
% \begin{figure}[!t]
%     \centering
%     \includegraphics[width=\linewidth]{figs/four_robot_three_object_hand_over-2.png}
%     \caption{Four-robot-in-line scene diagram of multi robot collaboration as image prompt transmitted to LLM planner. (the distance between each robot arm is 1m, and each arm's motion radius is about 0.8m)}
%     \label{fig:multi_arm_handover-line}
%     \vspace{-10pt}
% \end{figure}



 
% }

